IGB: Addressing The Gaps In Labeling, Features, Heterogeneity, and Size of Public Graph Datasets for Deep Learning Research

Graph neural networks (GNNs) have shown high potential for a variety of real-world, challenging applications, but one of the major obstacles in GNN research is the lack of large-scale flexible datasets. Most existing public datasets for GNNs are relatively small, which limits the ability of GNNs to generalize to unseen data. The few existing large-scale graph datasets provide very limited labeled data. This makes it difficult to determine if the GNN model's low accuracy for unseen data is inherently due to insufficient training data or if the model failed to generalize. Additionally, datasets used to train GNNs need to offer flexibility to enable a thorough study of the impact of various factors while training GNN models. In this work, we introduce the Illinois Graph Benchmark (IGB), a research dataset tool that the developers can use to train, scrutinize and systematically evaluate GNN models with high fidelity. IGB includes both homogeneous and heterogeneous academic graphs of enormous sizes, with more than 40% of their nodes labeled. Compared to the largest graph datasets publicly available, the IGB provides over 162X more labeled data for deep learning practitioners and developers to create and evaluate models with higher accuracy. The IGB dataset is a collection of academic graphs designed to be flexible, enabling the study of various GNN architectures, embedding generation techniques, and analyzing system performance issues for node classification tasks. IGB is open-sourced, supports DGL and PyG frameworks, and comes with releases of the raw text that we believe foster emerging language models and GNN research projects. An early public version of IGB is available at https://github.com/IllinoisGraphBenchmark/IGB-Datasets.

==> experiment.tex <==
%\clearpage
\section{Result}
\label{sec:result} 



% Baseline metrics. How to access the dataset, How we ran our stuff, Metrics and state about the dataset

% Hyperparameters go into the appendix. 

IGB provides five different sizes of datasets for model and system developers to work with. 
We evaluated IGB datasets on several different types of GNN models using the system described in $\S$~\ref{sec:syssetup}.
The high-level summary across GCN, GraphSage, and GAT models with a different number of output classes is provided in Table~\ref{table:model_perf}.

Apart from model accuracy for the IGB dataset, the work goal is also to study the impact of the dataset generation on GNN model accuracy. Our evaluation shows:  

\begin{itemize}
    \item Labeled data provides significant improvement in performance i.e., 150$\times$ more labeled data provides increases the node classification accuracy by up to ~10\%.
    \item Using an NLP model for initializing node embeddings is crucial as it provides over 40\% increase in GNN performance compared to randomly initialized embeddings.
    \item It is feasible to use dimensionality reduction algorithms like PCA to reduce the dimension of the node embedding by more than half and yet provide similar performance on the IGB dataset. 
    \item GNNs can play an important role in multilingual text embedding fine-tuning due to their reliance on structure and not the language.
\end{itemize}

\textbf{IGB-tiny t-SNE view:}
t-Distributed Stochastic Neighbor Embedding t-SNE~\cite{tsne} is an unsupervised method that can be used to perform dimensionality reduction by maximizing variance and preserving local similarities. This allows it to cluster similar embeddings closer while pushing dissimilar embeddings away providing a better visualization. We created a t-SNE representation of IGB-tiny to illustrate the graph is a 2D space with similar nodes clustered together. 

\subsection{Setup}
\label{sec:syssetup}
\begin{table}[!h]
% \vspace{3mm}
\centering
% \scriptsize
    % \vspace{-5ex}
    \caption{{System specification}}
    \begin{tabular}{|p{1in}|p{1.5in}|}
    \hline
    {\textbf{Configuration}}   & {\textbf{Specification}} \\
    \hline
    \hline
    {System}      &  { Supermicro AS-4124GS-TNR}   \\
    \hline
    {CPUs}         &  { 2$\times$ AMD EPYC 7702 64-Core Processors }\\
    \hline
    {DRAM}         &  { 1TB Micron DDR4-3200 }    \\
    \hline
    {GPU}         &  { NVIDIA A100-80GB PCIe}    \\
    \hline
    {SSDs}         &  { 8$\times$ Samsung 980pro}    \\
    \hline
    {Operating System}  & {Ubuntu 20.04 LTS} \\
    \hline 
    {CUDA Driver and Tools} & {NVIDIA Driver 470.82, CUDA Toolkit 11.4} \\
    \hline
\end{tabular}
\label{tab:softhardconfig}
% \vspace{-5ex}
\end{table}
All the models were trained on a system with $255$ AMD EPYC 7702 64-Core Processors and an NVIDIA A100-PCIE-40GB GPU. We used a docker container for training and testing and the image used is \url{nvcr.io/nvidia/pytorch:22.08-py3}. 
All the datasets were run on batched GCN, SAGE, and GAT models implemented using DGL primitives. 
Along with the dataset, we provide a DGL and PyG data loader\footnote{PyG data loader will be released soon}.
We used a batch size of $10,240$ in order to maximize GPU SM utilization and shared memory. 
All the runs use a $0.01$ learning rate.
IGB-tiny and IGB-small datasets are run on models with 2 layers with a hidden dimension of $128$ and for GAT there are $4$ heads.
All the other models have 2 layers with a hidden dimension of $16$ and 2 heads in the GAT model. 
IGB-tiny and IGB-small are trained for $15$ epochs while the larger models are trained for $3$ epochs.

\subsection{Impact Of Labelled Nodes}
\begin{figure}[h]
\includegraphics[width=8cm]{figures/node_label_exp.pdf}
    \centering
    \caption{Comparison of GNN model performance on IGB-tiny dataset with different fractions of labeled nodes to understand the effect of labeled nodes.}
        \label{fig:labelvariation}
\end{figure}
We motivated the importance of labeled data in $\S$\ref{sec:motivation}. 
In this section, we will evaluate the impact of labeled data on IGB datasets.
To perform this experiment, we created several sub-dataset with different fractions of labeled data.
GCN, Graph-SAGE, and GAT were then trained and evaluated on these various sub-datasets. 
Our expectation is the accuracy of the models should improve as we add more labeled data as the tasks are performed using supervised learning techniques. 
Figure~\ref{fig:labelvariation} shows the improvement in average GNN model accuracy observed when we vary the number of labeled nodes from 1 to $1/150$. 
As expected, across all models, we observe significant performance improvement (~10\%) as we add more labeled data. 

\begin{table}[!htp]
\centering
\small
\caption{GNN performance compared with the fraction of dataset labeled}
\label{table:label_exp}
\vspace{1em}{}
\begin{tabular}{lr|ccc} 
\toprule
Model & Fraction  & {GCN} & {SAGE} & {GAT}  \\
Dataset & Labeled & Test & Test & Test \\ 
\midrule
\texttt{IGB-tiny} & $1/10$  & $53.91$ &  $56.76$ &  $53.28$\\
$19$ classes      & $1/50$  & $53.16$ &  $55.79$ &  $53.10$\\
                 & $1/100$  & $52.77$ &  $55.21$ &  $51.68$\\
                 & $1/150$  & $51.46$ &  $53.97$ &  $50.12$\\
                 \hline
\texttt{IGB-small} & $1/10$    & $69.25$ & $72.89$ & $68.76$\\
$19$ classes       & $1/50$    & $62.80$ & $65.88$ & $57.60$\\
                   & $1/100$   & $56.60$ & $57.00$ & $55.25$\\
                   & $1/150$   & $57.80$ & $56.30$ & $52.85$\\
\bottomrule
\end{tabular}
\end{table}

To validate the experimental results that can be extrapolated to the larger IGB datasets, we created two sub-variant of the dataset for \texttt{IGB-small} and \texttt{IGB-medium} and varied the number of labeled nodes from $1$ to $1/150$. 
We evaluated the performance improvement using the 3 models and then took the average. From Table~\ref{table:fractiondataset} we see that there is a steady decrease in the difference between the accuracy of the full dataset and that of the 1/250 fraction. 
This is because, as the dataset increases in size, the models can learn more from the structure and depends less on the labeled nodes.
As expected, a similar performance improvement was noted. 
This shows that we can theoretically extrapolate this difference to the large and full model as well, showing a significant bump in test accuracy over datasets with much less labeled data. 
Additionally, with more labeled data we can finally use the whole dataset for training which allows us to work on the GNN training speed and test architectural inefficiencies. 


\begin{table}[htp]
\centering
\tiny
\caption{Node label experiment on various IGB datasets taking an average of GCN, SAGE, and GAT to compare the accuracy difference between the full labeled dataset and 1/150 of the dataset.}
\label{table:fractiondataset}
\vspace{1em}{}
\begin{tabular}{lcc|r} 
\toprule
Dataset & Full-labelled acc & ${1}/{150}$ labelled acc & Difference \\ 
\midrule
\texttt{IGB-tiny} & $69.62\%$ & $51.85\%$ & $17.77$ \\
\texttt{IGB-small} & $72.28\%$ & $55.65\%$ & $16.63$ \\
\texttt{IGB-medium*} & $70.34\%$ & $58.15\%$ & $12.18$ \\
% \hline
% & & Average & \boldmath{$16.10\pm2.42$}\\
\hline
\end{tabular}
\end{table}


\subsection{Impact Of Node Embedding Generation}
We will study the effect of node embeddings on GNN accuracy and the impact of embedding dimension, generation model, and language in this section. 

\textbf{Importance Of Embeddings From Large Language Models }
In order to provide the GNN model with information about the node itself, we need to initialize each node with representative embeddings. 
Of course, the question arises what happens if we initialize the embeddings with random vectors. 
Our evaluation shows that the difference in GNN performance with random embeddings and NLP-based embeddings is very stark. 

We ran IGB-tiny, small, and medium with roberta (1024-dim) embeddings and random embeddings to compare the difference in test accuracy. 
Using the large language models for embeddings increases the model performance by more than 3$\times$ in the IGB-tiny, IGB-small, and IGB-medium. 
Extrapolating this, we can predict that this holds for IGB-large and IGB260M too since without the NLP node embeddings the GNN doesn't have any information about the node so it can only learn from the graph structure.

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{figures/node_rand_exp.pdf}
\caption{Random vs 1024-dim NLP embeddings affecting average GNN performance in IGB-tiny, IGB-small, and IGB-medium.}
\end{figure}

\begin{table}[htp]
\caption{GNN performance compared with random embeddings vs $1024-dim$ embeddings}
\centering
\tiny
\vspace{1em}{}
\begin{tabular}{lccccccc} 
\toprule
Model & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{SAGE} & \multicolumn{2}{c}{GAT}  \\
Dataset &  random & real & random & real & random & real \\ 
\midrule
\texttt{IGB-tiny} & & & & & \\
19 classes & $25.09$ & $68.06$ & $25.37$ & $71.87$ & $27.10$ & $68.92$ \\
2983 classes & $23.49$ & $53.13$ & $22.29$ & $59.49$ & $23.29$ & $51.74$ \\
\hline
\texttt{IGB-small} & & & & & \\
19 classes & $26.02$ & $70.46$ & $25.17$ & $75.49$ & $27.46$ & $70.93$ \\
2983 classes & $23.88$ & $63.28$ & $23.38$ & $68.70$ & $24.88$ & $63.70$ \\
\bottomrule
\end{tabular}
\label{table:label_exp}
\end{table}

\textbf{Selecting Right Embedding Model }
In order to understand the effect of various large generic language models, we evaluated GNN model accuracy with a few widely used sentence transformer models from the Huggingface library~\cite{huggingface}. Table~\ref{tab:nlpmodels} summarizes the reported average performance on NLP tasks and model size of generic language models along with their embedding dimensions. 


\begin{table}[htp]
\centering
\caption{Sentence Transformer Models from the Huggingface Library}
\tiny
\vspace{1em}{}
\begin{tabular}{lrrr} 
\toprule
Dataset & Emb dim & Avg. perf & Model size \\ 
\midrule
\texttt{all-MiniLM-L6-v2} & $384$ & $58.80\%$ & $80$ MB \\
\texttt{distiluse-base-multilingual} & $512$ & $45.59\%$ & $480$ MB \\
\texttt{all-mpnet-base-v2} & $768$ & $63.30\%$ & $420$ MB \\
\texttt{all-roberta-large-v1} & $1,024$ & $61.64\%$ & $1,360$ MB \\
\bottomrule
\end{tabular}
\label{tab:nlpmodels}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{figures/diff_nlp_model.pdf}
    \caption{GNN accuracy on IGB-tiny using different NLP embedding models for initializing node embeddings.}
    \label{fig:embeddmodel}
\end{figure}

Figure~\ref{fig:embeddmodel} summarizes the impact of different language models on the GNN accuracy by taking the average of GCN, GraphSAGE, and GAT to get model-independent trends.
As the embedding dimensions are different, it is impossible to conclude if such a large performance range is due to the model's accuracy or embedding dimensions.
However, what can be concluded is that the NLP model in itself has a direct impact on the GNN performance.
In the next experiment, we will isolate the impact of the model by normalizing the embedding dimensions using the dimensionality reduction technique. 
As the embedding dimensions are not the same, it is hard to determine if the model played the role or if the additional information learned by the model by having a larger footprint helped in increasing the accuracy.

\textbf{Impact Of Embedding Dimension }
The previous experiment compared different-sized embeddings from various NLP models. To understand how the models affect the performance we must normalize the embedding dimensions. For models with higher dimensions, we used the dimensionality reduction technique, principle decomposition analysis (PCA)~\cite{pca}, and normalized the embedding dimensions. We used the GPU implementation of PCA from the cuML API library~\cite{cuml}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{figures/node_emb_exp.pdf}
    \caption{Average GNN performance on IGB-tiny based on NLP embedding model after PCA.}
    \label{fig:dimstudy}
\end{figure}

\begin{table*}[!htp]
\caption{GNN performance on IGB-tiny NLP model after PCA dim reduction. The x rows represent the original NLP model dimension and the columns represent the final emb dimension after PCA reduction.}

\centering
\begin{tabular}{l|c@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}c|c@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}c|c@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}c} 
\toprule
& \multicolumn{4}{|c|}{GCN} & \multicolumn{4}{|c|}{SAGE} & \multicolumn{4}{|c}{GAT} \\
Dimension & 384 & 512 & 768 & 1024 & 384 & 512 & 768 & 1024 & 384 & 512 & 768 & 1024 \\ 
\midrule
miniLM-384 & $66.33$ & - & - & - & $70.57$ & - & - & - & $67.60$ & - & - & -  \\
DISTILUSE-512 & $58.21$ & $64.51$ & - & - & $64.98$ & $68.03$ & - & - & $63.03$ & $65.09$ & - & - \\
MPNET-768 & $62.30$ & $63.10$ & $67.79$ & - & $68.54$ & $69.27$ & $71.24$ & - & $65.95$ & $66.17$ & $68.26$ & - \\ 
ROBERTA-1024& $60.90$ & $62.52$ & $62.94$ & $68.06$ & $68.73$ & $69.48$ & $70.00$ & $71.87$ & $65.64$ & $65.92$ & $66.15$ & $68.92$ \\ 
\bottomrule
\end{tabular}
\label{table:nlp_diff_emb_exp}
\end{table*}

We ran IGB-tiny with all the possible combinations of dimensions using GCN, GraphSAGE, and GAT GNNs models, and the results are described in Table~\ref{table:nlp_diff_emb_exp}. 
Reducing the dimensions of embeddings using PCA impacts the GNN model accuracy across all GNN models. 
This is nothing surprising as the PCA is a lossy operation. 
For Roberta embeddings, when the embedding dimensions are reduced from 1024 to 384, we observe 3.55\%, 1.47\%, and 0.58\% reduction in accuracy for GCN, GraphSAGE, and GAT GNN models. 
A similar observation is noted in the case of mpnet embeddings and others. 
This is interesting because from the data we note that the GAT GNN model is more resilient to embedding dimension reductions compared to the GraphSAGE and GCN models. 

Moreover, for Roberta embeddings, 2.6$\times$ reduction in embedding dimension only resulted in up to 3.55\% accuracy loss in the GNN models on the IGB-tiny datasets. 
This is important as 1024-dim embeddings consume massive memory capacity for storing embeddings vectors during training and inference operations and 2.6$\times$ is a significant cost saving especially for IGB260 full. 
Obviously, the next question is, can we save more memory by further reducing the dimensionality. 
To understand this, we reduced the embedding dimensions from 1023 to 8 using PCA and evaluate different GNN model accuracies for Roberta embedding vectors as shown in Figure~\ref{fig:extremedimstudy}. 

Reducing the embedding dimension by 2$\times$ results in 1.03\%, 0.72\%, and 0.30\% reduction in accuracy for GCN, GraphSAGE, and GAT GNN models. 
Projecting this to $IGB260M$ dataset translates to about a 50\% reduction in memory space required for running these models. 
Further reducing the embedding dimensions deteriorates the performance of GNN models. 
With embedding dimensions of 128 and 8, the accuracy drops by 4.1\%, 3.39\%, 2.17\% and 13.41\%, 12.24\%, 9.35\% for GCN, GraphSAGE, and GAT GNN models respectively.  

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{figures/emb_dim_extreme.pdf}
    \caption{GNN performance on Roberta embeddings from 1024-dim to 8-dim across all GNN models}
        \label{fig:extremedimstudy}
\end{figure}


Figure~\ref{fig:dimstudy} captures the average of three GNN model accuracy for the IGB-tiny dataset for all NLP embeddings when their embedding dimensions are normalized. 
The mpnet and Roberta outperform the other miniLM and distiluse models across all GNN models. 
This is because both these NLP models used for embedding generations inherently are better at language modeling tasks (see Table~\ref{tab:nlpmodels} and thus their respective accuracy improvements also get reflected in the GNN model's accuracy. 
This is good as it aligns with the industrial trend towards building more accurate generic foundational language models which can further improve the GNN model performance. 


Based on this analysis, by default, IGB provides 1024-dim Roberta embeddings vectors which can be converted using the provided toolchains in the IGB dataset. Interested users who want to generate embeddings using other models, can easily generate them by using the tools provided in our open-source codebase~\cite{igb260m}.

\subsection{Language Influence On Embeddings}
Often large language models (LLMs) are trained on web corpus data~\cite{gpt2, roberta}. 
The majority of the data used for training NLP models are in the English language and thus the embedding generated can have a bias towards a specific language.  
The MAG dataset used to generate the IGB dataset comprises more than 80 languages of papers. More than 12 languages have over 1M nodes and 50\% of nodes have English papers in the MAG dataset as shown in Figure~\ref{fig:langdist}.
Thus, it is of utmost importance to understand if the language in which LLMs are trained matters on the overall accuracy of the GNN models. 
\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{figures/paper_lang.pdf}
    \caption{Paper language distribution in the MAG database}
    \label{fig:langdist}
\end{figure}
Our goal is to determine if the language used in the dataset to train the NLP model makes any difference in the GNN performance.
To do this, we must use the NLP model trained exclusively on a specific language.
However, finding a pre-trained large language model exclusively on a specific language is nearly impossible as of today and thus, we ended up using multilingual language models that include or exclude specific language for this experiment. 
We picked three languages Japanese, Spanish and French in our study and created sub-datasets by generating node embeddings with the pre-trained multilingual models from the HuggingFace repository~\cite{huggingface}.  The models used are: \\
\textbf{\texttt{paraphrase-MiniLM-L12-v2 }: (384-eng)} \small{Trained on only English with 384 embedding dimensions.}\\
\textbf{\texttt{paraphrase-multilingual-MiniLM-L12-v2 }: (384-all)} \small{Multilingual version of paraphrase-MiniLM-L12-v2, trained on parallel data for 50+ languages and producing 384-embedding dimensions.}\\
\textbf{\texttt{paraphrase-mpnet-base-v2 }: (768-eng)} \small{Trained on only English. The embedding dimensions are 768.}\\
\textbf{\texttt{paraphrase-multilingual-mpnet-base-v2 }: (768-all)} \small{Multilingual version of paraphrase-MiniLM-L12-v2, trained on parallel data for 50+ languages including English. The embedding dimensions are 768. This includes Japanese.}\\
\textbf{\texttt{distiluse-base-multilingual-cased-v1}: (512-v1)} \small{Multilingual knowledge distilled version of multilingual Universal Sentence Encoder. Supports 13 languages: Arabic, Chinese, Dutch, English, French, German, Italian, Korean, Polish, Portuguese, Russian, Spanish, and Turkish. The embedding dimensions are 512.}\\
\textbf{\texttt{distiluse-base-multilingual-cased-v2}: (512-v2)} \small{Multilingual knowledge distilled version of multilingual Universal Sentence Encoder. This version supports 50+ languages. The embedding dimensions are 512.}

We generated two types of embeddings, one with the NLP model trained in the English language (english embedding) and the other with the NLP model trained on multi-lingual that includes Japanese/Spanish/French (multi-lingual embedding). 
The final created dataset properties are shown in Table~\ref{tab:langigbdataset}.

\begin{table}[htp]
\centering
\caption{Test datasets created from IGB based on 3 different languages.}
\tiny
\begin{tabular}{lrrr} 
\toprule
Dataset & \#Nodes & \#Edges &  Emb-dim \\ 
\midrule
\texttt{IGB-japanese} & $1,975,296$ & $3,291,665$ & $384/512/768$ \\
\texttt{IGB-spanish} & $1,207,296$ & $1,266,183$ & $384/512/768$  \\
\texttt{IGB-french} & $841,728$ & $1,688,202$ & $384/512/768$ \\
\bottomrule
\end{tabular}
\label{tab:langigbdataset}
\end{table}
\begin{table}[htp]
\centering
\tiny
\caption{Performance of average GNN model with different languages showing that language doesn't affect GNN model accuracy significantly}
\begin{tabular}{lrrr} 
\toprule
Model* & \texttt{IGB-japanese} & \texttt{IGB-spanish} &  \texttt{IGB-french} \\ 
\midrule
$384-eng$ & $62.89$ & $59.77$ & $60.39$ \\
$384-all$ & $62.83$ & $59.01$ & $59.48$ \\
\hline
Average & \boldmath{$62.86_{\pm0.03}$} &  \boldmath{$59.39_{\pm0.38}$} &  \boldmath{$59.94_{\pm0.46}$} \\
\hline
$768-eng$ & $64.82$ & $61.63$ & $61.15$  \\
$768-all$ & $64.74$ & $61.77$ & $61.25$  \\
\hline
Average & \boldmath{$64.78_{\pm0.04}$} &  \boldmath{$61.70_{\pm0.07}$} &  \boldmath{$61.20_{\pm0.05}$} \\
\hline
$512-v1$ & $61.82$ & $58.86$ & $57.48$  \\
$512-v2$ & $61.61$ & $58.42$ & $57.04$  \\
\hline
Average & \boldmath{$61.72_{\pm0.11}$} &  \boldmath{$58.64_{\pm0.22}$} &  \boldmath{$57.26_{\pm0.22}$} \\
\bottomrule
\end{tabular}
%*\url{https://www.sbert.net/docs/pretrained_models.html#sentence-embedding-models/}%
\label{tab:langperf}
\end{table}

Table~\ref{tab:langperf} shows the performance achieved by averaged GNN model with {english-embedding} and {multi-lingual-embedding}.  
From Table~\ref{tab:langperf}\footnote{We also normalized the embedding dimensions using PCA and did not notice a difference in the trend.}, irrespective of model dimensions and NLP model, there is no significant performance improvement achieved by including specific language of interest.
To confirm that this isn't a language-dependent artifact we ran different embedding dimension models on the French and Spanish datasets and noticed a similar trend on GCN, graphSAGE, and GAT. 
We believe this is because the GNNs learn from the structure of the graph whereas the NLP models rely on the provided text information. 
Because of this unique ability, GNN models can become language agnostic and help in making NLP models better. 


\subsection{Limitations In Existing Systems And Framework}
IGB is the largest GNN dataset publicly available as of today. The full dataset consumes over 1.2TB in space and due to this, many systems fail to adequately support efficient training and inferencing.
In this section, we will describe the problems that we encountered while running IGB on state-of-the-art systems and describe potential solutions to the problem. 

IGB260M consists of 269+M nodes with 1K-dim embedding vectors in single precision representation requiring more than 1TB of memory capacity in a single node. 
This memory capacity requirement of IGB260M exceeds the host memory capacity available in modern high-end data center single node-servers. 
This makes the training within a node infeasible. 
To address this, one can memory-map the embedding vectors and keep the embedding vectors in a fast-storage medium like SSDs. 
This enables frameworks like DGL to work on embedding tables that exceed host memory in a single node. 
One can enable this using Numpy~\cite{numpy} memory-map abstraction. 

Although the memory-map abstraction enables training or inferencing to execute on a single node, the entire execution becomes slow when compared to host-memory execution. 
This is because the memory-map abstraction uses a page-fault mechanism to generate a read request to the storage and move the embedding vectors from storage to CPU memory and then to GPU memory. 
This incurs significant overhead and overall execution time increases dramatically reducing average GPU utilization as shown in Figure~\ref{fig:gpuutilfull}\footnote{GPU utilization is captured using \texttt{nvidia-smi} tool over a period of 1800 seconds with one second sampling frequency.}. 


\begin{figure}[h]
    \includegraphics[width=8cm]{figures/full_gpu_stats.png}
    \centering
    \caption{GPU streaming multiprocessor utilization for IGB.}
    \label{fig:gpuutilfull}
\end{figure}

If the model fits in the host memory as in the case of IGB-large, then the GPU utilization is significantly improved and reached up to 80\%. Here, our codebase exploits the DGL-UVA~\cite{emogi, pytorchdirect} techniques where the GPU can directly sample the embedding vectors stored in the CPU memory. 
This helps to improve the overall training execution time. 
However, there are still time periods in the training iteration when the GPU utilization is not reaching a peak and is mainly limited by the CPU throughput. 
This requires further profiling and analysis which we leave as future work.

If the model fits in the GPU memory, as in the case of IGB-tiny, we can train the entire model in 120 seconds and the average GPU utilization is high.
This is because embeddings tables can be directly accessed which increases the average GPU utilization. 
Thus, enabling efficient embeddings gather operation is fundamental to the performance of the GNN training algorithm.
Hence, from the programmer's perspective, depending on the model size, the GNN model developer must make necessary changes to the source code to ensure it fits in the respective memory hierarchy for efficient execution. 
However, ideally, what GNN model developers require is a way to efficiently execute GNN models using a single embedding loader class for the IGB dataset that is memory-hierarchy aware and can provide the best performance based on where the embedding vectors are.
Such a system design is beyond the scope of this work and leave as future work.

Furthermore, as the graph size increases, the system requires to evolve and support efficient access to gather embedding vector from wherever it is stored, be it in memory or storage. 
However, current system designs are focused exclusively on how to improve performance while gathering data from memory. 
More recently, the works like BaM~\cite{bamarxiv, vikramwork, zaidwork} can help address this gap directly where the GPU threads can directly read the data where it is stored. 
How one can integrate BaM into frameworks like DGL while running the IGB dataset is beyond the scope of the work and left as future work. 

\begin{figure}[h]
    \includegraphics[width=8cm]{figures/tiny_gpu_stats.png}
    \centering
    \caption{GPU streaming multiprocessor utilization for IGB-tiny.}
    \label{fig:gpuutilfull}
\end{figure}

In this work, we focused on single-node GNN model training. 
We did not evaluate multi-node and multi-GPU training and inferencing due to the lack of system availability and the complexity involved. 
We hope to address them in the future. 



\section{IGB Dataset Model Perf Summary}


\begin{table*}[htp]
\centering
\caption{IGB Datasets homogeneous benchmark using same model size all the datasets (* trained for 3 epochs)}
\begin{tabular}{lcccccc} 
\toprule
Model & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{SAGE} & \multicolumn{2}{c}{GAT} \\
Dataset & 19 acc & 2983 acc &  19 acc & 2983 acc & 19 acc & 2983 acc \\ 
\midrule
\texttt{IGB-tiny} & $68.06$ & $53.13$ & $71.87$ & $59.49$ & $68.92$ & $51.74$\\
\texttt{IGB-small} & $70.46$ & $63.28$ & $75.49$ & $68.70$ & $70.93$ & $63.70$\\
\hline
\texttt{IGB-medium*} & $70.63$ & $62.70$ & $70.35$ & $62.55$ & $70.06$ & $61.81$\\
\texttt{IGB-large*} & $50.29$ & $-$ & $64.89$ & $-$ & $64.59$ & $-$\\
\texttt{IGB260M*} & $48.59$ & $-$ & $54.95$ & $-$ & $55.51$ & $-$\\
\bottomrule
\end{tabular}
\label{table:model_perf_repeat}
\end{table*}

In this section, we will summarize the overall results of IGB datasets across all the GNN models and two different complex tasks as shown in Table~\ref{table:model_perf_repeat}.
The IGB-tiny and small have each been trained for $20$ epochs with the $19$ and $2983$ class tasks using GCN, GAT, and GraphSAGE GNN models. 
The accuracy of the models generally sees a dip in performance in the $2983$ class task due to the additional complexity of the task where the model has to find a finer difference in the nodes to classify them into a such large number of classes. 
Increasing the class tasks from 19 to 2983 sees a drop in performance by 14.93\%, 12.38\%, and 17.18\% in GCN, SAGE, and GAT respectively, and 7.18\%, 6.79\%, and 7.23\% in GCN, SAGE and GAT respectively. 
Some of these accuracies drop can be recovered by training for longer epochs. 
However, fundamentally, better models are required to predict fine-class tasks.

The IGB-small dataset is the most similar in terms of size to the homogeneous version of MAG240M~\cite{ogbn-mag}.
In terms of performance, they also closely correlate as both have been curated with similar input data~\cite{ogbn-mag}.
IGB-medium and the larger models have been trained for $3$ epochs each with all three models. 
IGB-large and full are currently extremely hard to train in the available hardware resources at our disposal.  
We could train for three epochs with 19 out-class tasks. 
However, training 2983 class tasks in a single node system requires system innovations. 







==> relatedwork.tex <==
\section{Related work}

% vikram

% \label{sec:background}

% I'm citing ~\cite{aifb}

% \cite{FakeNewsDataset}

% Para 1: Citing all the previous datasets about GNN (general)

% Para 2: Large graphs in GNN community

% table

% Para 3: Limitation of current datasets

% Para 4: Graph datasets for system study (if doesn't exist say doesn't exist our graph asks this question)

% Para 5: Labels (Find papers which say not many labels) and embeddings generation (how other papers generate it and why this isn't cool since they only test one emb size)


\label{sec:dataset}
In $\S$~\ref{sec:graphneuralnet} we discussed the most popular supervised GNN models. Supervised learning models require data with ground truth labels which can be used for training and setting up test benchmarks. 
Furthermore, understanding graph structure greatly helps to understand model performance. 
Thus, it is essential to define the commonly used metrics while studying the graph structure relevant to GNN. Although these metrics are comprehensive, it provides sufficient details to help understand GNN model accuracy. 
The most important metric for each dataset is the number of nodes/edges, the number of classes, and node embedding dimensions. These metrics allow us to determine the scale of GNN models and the expressiveness of the input data. 
Average degree distribution can also be easily calculated from the specified information.
Apart from these metrics, homophily $(\beta)$ for a graph is a very important metric as shown by many researchers.\cite{homophily_effects}.
Homophily is defined as the fraction of neighbors for each node in a graph with the same label as that node itself~\cite{homophily}. This can be represented in an equation as,
\begin{equation}
    \beta = \frac{1}{|V|} \sum_{v \in V} \frac{\#\{n_u : \mathcal{L}(n_u) == \mathcal{L}(n_v), u \in \mathcal{N}(v)\}}{\#\{n_u : u \in \mathcal{N}(v)\}}
\end{equation}
where $V$ is the total number of nodes in the graph and $\mathcal{L}(x)$ is the label of node $x$. 

Apart from homophily, the number of connected components directly affects the performance of GNN models on dataset~\cite{homophily_effects, cc_graph_perf}. As this work proposes a new dataset for GNN, we must compare eventually to understand how these metrics stand across different graph datasets. 

The Open Graph Benchmark (OGB) and Deep Graph Library (DGL) have a set of graph datasets for various types of GNN tasks like node/graph classification and edge prediction. 
These sources provide easy access to data loaders for these datasets and also include benchmarks and leaderboards. Some of the popular node classification graph datasets are~\cite{citeseer, coragraph, snap} listed along with their  metrics in Table~\ref{table:popular_node_classification_datasets}.
\begin{table*}[h]
\centering
% Number of classes, Connected Comp, Triangle Count, Embedding shape
\caption{Popular node classification datasets}
\begin{tabular}{lrrrr} 
\toprule
Dataset & \#Nodes & \#Labelled & \#Edges & Homophily  \\ 
\midrule
\texttt{citeseer} & $3,327$ & $1,620$ & $9,228$ & 73.91\% \\
\texttt{pubmed} & $19,717$ & $2,100$ & $88,651$ & 80.24\% \\
\texttt{cora} & $19,793$ & $19,793$ & $126,842$ & 81.00\% \\
\texttt{ogbn-arxiv} & $169,343$ & $169,343$ & $1,166,243$ & 65.51\% \\
\texttt{ogbn-mag} & $1,939,743$ & $736,389$ & $21,111,007$ & 30.40\% \\
\texttt{ogbn-papers100M} & $111,059,956$ & $~1,500,000$ & $1,615,685,872$ & - \\
\texttt{mag-240m~\cite{ogblsc}} & $121,751,666$ & $~1,400,000$ & $1,297,748,926$ & - \\
\bottomrule
\end{tabular}
\label{default}
\end{table*}

\begin{table*}[htp]
\centering
\caption{Popular node classification datasets metrics.}
\begin{tabular}{lrrrr} 
\toprule
Dataset & \#Classes & Emb & Connected Comp  \\ 
\midrule
\texttt{citeseer} & $6$ & $3,703$ & $438$ \\
\texttt{pubmed} & $3$ & $500$ & $1$ \\
\texttt{cora} & $70$ & $8,710$ & $78$ \\
\texttt{ogbn-arxiv} & $40$ & $128$ & $1$ \\
\texttt{ogbn-mag} & $349$ & $128$ & $3,798$ \\
\texttt{ogbn-papers100M} & $172$ & $128$ & - \\
\texttt{mag-240m~\cite{ogblsc}} & $153$ & $768$ & - \\
\bottomrule
\end{tabular}
\label{table:popular_node_classification_datasets}
\end{table*}

